How Many Topics? Stability Analysis for Topic Models

Topic modeling refers to the task of discovering the underlying thematic structure in a text corpus, where the output is commonly presented as a report of the top terms appearing in each topic. Despite the diversity of topic modeling algorithms that have been proposed, a common challenge in successfully applying these techniques is the selection of an appropriate number of topics for a given corpus. Choosing too few topics will produce results that are overly broad, while choosing too many will result in the "over-clustering" of a corpus into many small, highly-similar topics. In this paper, we propose a term-centric stability analysis strategy to address this issue, the idea being that a model with an appropriate number of topics will be more robust to perturbations in the data. Using a topic modeling approach based on matrix factorization, evaluations performed on a range of corpora show that this strategy can successfully guide the model selection process.

==> data_full.tex <==
%!TEX root = ecml14topic.tex
\section{Evaluation}
\label{sec:eval}

\subsection{Data}

We now evaluate the stability analysis approach described in \refsec{sec:methods} to assess its usefulness in guiding the selection of the number of topics. The evaluation is performed on a number of text corpora, each of which has annotated ``ground truth'' document labels such that each document is assigned a single label:
\begin{itemize}
\item \emph{bbc}: A corpus of news articles from the BBC that has previously been used for document clustering \cite{greene05pkdd}. Articles are divided into five topical areas: business, entertainment, politics, sport, technology 
\item \emph{bbc-sport}: A smaller set of news articles from the BBC, relating to five different sports: athletics, cricket, football, rugby, tennis.
\cite{greene05pkdd}.
\item \emph{guardian-2013}: A new corpus of news articles published by The Guardian during 2013. Article labels are assigned based on the section in which it appeared on the website: books, business, fashion, football, music, politics.
\item \emph{irishtimes-2013}: Another selection of news articles from 2013, this time published by The Irish Times. Again disjoint labels were assigned based on section assignment on their website (\eg economy, health, politics).
%: crime \& law, economy, golf, health, politics, rugby, soccer.
\item \emph{nytimes-1999}: A subset of the New York Times Annotated Corpus, which has previously been used for LDA topic modeling experiments \cite{sandhaus08nytimes}. This subset covers articles published in 1999 belonging to one of the following categories: business, education, health, sports.
\item \emph{nytimes-2003}: A corpus generated from the same source as above, with articles published in 2003 belonging to one of seven categories: business,  automobiles,  education, dining \& wine, health, movies, sports.
\item \emph{wikipedia-high}: A sample of a complete dump of Wikipedia retrieved in January 2014, where articles are assigned one of six labels based on their high level WikiProject\footnote{See \url{http://en.wikipedia.org/wiki/Wikipedia:WikiProject}} categorization (\eg music, sports).
%: medicine, military \& warfare, music, space, sports, transportation.
\item \emph{wikipedia-low}: A corpus generated from the same source as above, but where articles are assigned one of ten labels based on more fine-grained WikiProject sub-groups (\eg automobile, jazz, opera).
\end{itemize}
%
When pre-processing each corpus, terms occurring in $< 20$ documents were removed, along with English language stop words, but no stemming was performed. Standard log TF-IDF and unit length normalization procedures were then applied to the term-document matrix. Details of the corpora are reported in \reftab{tab:data}, and pre-processed versions are made available online for further research\footnote{\url{http://mlg.ucd.ie/howmanytopics/}}.

\begin{table}[!t]
	\centering
    \caption{Details of the corpora used in our experiments, including the number of labels in the associated ``ground truth'' categorization scheme.}
    \label{tab:data}
    \begin{tabular}{|p{2.8cm}|c|c|c|}
    \hline
    \emph{Corpus}             & \emph{Documents} & \;\;\emph{Terms}\;\; & \;\emph{\# Labels}\; \\
    \hline
    bbc                 & 2225     & 3121     & 5  \\
    bbc-sport            & 737      & 969      & 5  \\
    guardian-2013   	& 6520     & 10801    & 6  \\
    irishtimes-2013    & 3246     & 4832     & 7  \\
	nytimes-1999            & 9551     & 12987     & 4  \\
    nytimes-2003            & 11527     & 15001     & 7  \\
    wikipedia-high      & 5738     & 17311    & 6  \\
    wikipedia-low       & 4986     & 15441    & 10 \\
    \hline
    \end{tabular}
\end{table}


\begin{table}[!t]
	\centering
	\begin{tabular}{|l|c|c|}\hline
\emph{Measure}          & \emph{Mean Variance} & \emph{Mean Std.} \\ \hline
Consensus        & 0.000         & 0.015     \\
Stability $(t=10)$ & 0.004         & 0.066     \\
Stability $(t=20)$                & 0.005         & 0.068     \\
Stability $(t=50)$    & 0.005         & 0.070     \\
Stability $(t=100)$\;\;\;    & 0.005         & 0.069    \\\hline
\end{tabular}
\end{table}
